Constrained and unconstrained stable discrete minimizations for p-robust local reconstructions in vertex patches in the de Rham complex

We analyze constrained and unconstrained minimization problems on patches of tetrahedra sharing a common vertex with discontinuous piecewise polynomial data of degree p. We show that the discrete minimizers in the spaces of piecewise polynomials of degree p conforming in the H1, H(curl), or H(div) spaces are as good as the minimizers in these entire (infinite-dimensional) Sobolev spaces, up to a constant that is independent of p. These results are useful in the analysis and design of finite element methods, namely for devising stable local commuting projectors and establishing local-best/global-best equivalences in a priori analysis and in the context of a posteriori error estimation. Unconstrained minimization in H1 and constrained minimization in H(div) have been previously treated in the literature. Along with improvement of the results in the H1 and H(div) cases, our key contribution is the treatment of the H(curl) framework. This enables us to cover the whole De Rham diagram in three space dimensions in a single setting.

==> figure_mixed_patches.tex <==
\tikzset{math3d/.style=
{x= {(-0.353cm,-0.353cm)}, z={(0cm,1.3cm)},y={(0.0cm,0.7cm)}}}
%{x= {(-0.5cm,-0.5cm)}, z={(0cm,1.0cm)},y={(0.0cm,0.5cm)}}}

\begin{figure}
\def\sz{0.65}
\def\sza{0.45}
\def\opac{1}

\begin{minipage}{.45\linewidth}
\centering
\begin{tikzpicture}[math3d, scale=3.3]
%filled faces
\fill[color=gray!20] (0,0, 1) -- (-1,-1,0) -- (0,0,0) -- cycle;
\fill[color=gray!20] (0,0,-1) -- (-1,-1,0) -- (0,0,0) -- cycle;
\fill[color=gray!20] (0,0, 1) -- ( 1, 1,0) -- (0,0,0) -- cycle;
\fill[color=gray!80] (0,0,-1) -- ( 1, 1,0) -- (0,0,0) -- cycle;

%edges
\draw[        line width=\sz pt] (-1,-1,0)--(0,0,0)--(1,1,0);

\draw[        line width=\sz pt] ( 0, 0, 0) -- ( 0, 0, 1);

\draw[dashed, line width=\sz pt] ( 1, 1, 0) -- (-1, 0, 0);
\draw[        line width=\sz pt] (-1,-1, 0) -- (-1, 0, 0);
\draw[        line width=\sz pt] ( 0, 0, 1) -- (-1, 0, 0);
\draw[dashed, line width=\sz pt] ( 0, 0, 0) -- (-1, 0, 0);
\draw[dashed, line width=\sz pt] ( 0, 0,-1) -- (-1, 0, 0);

\draw[        line width=\sz pt] ( 0, 0, 1) -- ( 1, 1, 0);
\draw[        line width=\sz pt] ( 0, 0, 1) -- (-1,-1, 0);

\draw[        line width=\sz pt] ( 0, 0, 0) -- ( 0, 0,-1);
\draw[        line width=\sz pt] ( 0, 0,-1) -- ( 1, 1, 0);
\draw[        line width=\sz pt] ( 0, 0,-1) -- (-1,-1, 0);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.45\linewidth}
\centering
\begin{tikzpicture}[math3d, scale=3.3]
%filled faces
\fill[color=gray!20] (-1, 0, 0) -- (-1, 0,-1) -- (0,0,0) -- cycle;
\fill[color=gray!20] ( 0, 0,-1) -- (-1, 0,-1) -- (0,0,0) -- cycle;
\fill[color=gray!80] ( 0, 0,-1) -- ( 1, 1, 0) -- (0,0,0) -- cycle;
\fill[color=gray!20] (-1, 0, 0) -- ( 1, 1, 0) -- (0,0,0) -- cycle;

\draw[line width=\sz pt] (-1, 0, 0) -- (-1, 0,-1) -- (0,0,0) -- cycle;
\draw[line width=\sz pt] ( 0, 0,-1) -- (-1, 0,-1) -- (0,0,0) -- cycle;
\draw[line width=\sz pt] ( 0, 0,-1) -- ( 1, 1, 0) -- (0,0,0) -- cycle;
\draw[line width=\sz pt] (-1, 0, 0) -- ( 1, 1, 0) -- (0,0,0) -- cycle;

\draw[dashed,line width=\sz pt] (-1, 0, 0) -- (-0.3,1,-1);
\draw[dashed,line width=\sz pt] ( 0, 0,-1) -- (-0.3,1,-1);
\draw[dashed,line width=\sz pt] ( 0, 0,-1) -- (-0.3,1,-1);
\draw[dashed,line width=\sz pt] (-1, 0, 0) -- (-0.3,1,-1);

\draw[dashed,line width=\sz pt] (-1, 0,-1) -- (-0.3,1,-1);
\draw[dashed,line width=\sz pt] (-1, 0,-1) -- (-0.3,1,-1);
\draw[dashed,line width=\sz pt] ( 1, 1, 0) -- (-0.3,1,-1);
\draw[dashed,line width=\sz pt] ( 1, 1, 0) -- (-0.3,1,-1);

\draw[dashed,line width=\sz pt] ( 0, 0, 0) -- (-0.3,1,-1);
\end{tikzpicture}
\end{minipage}

\caption{Example of patches with mixed boundary conditions covered by Theorem~\ref{thm_mixed}.
The original patch is on the left and its bilipschitz mapping on the right. If the
dark grey boundary correspond to $\Ga$ (and thus, the light grey is $\FDa$), then
the deformed patch fits the setting of Lemma~\ref{lemma_mixed_planar}. Conversely,
if the light grey represents $\Ga$ (and the dark grey $\FDa$), then the bilipschitz
mapped patch is covered by Lemma \ref{lemma_mixed_wedge}.}
\label{figure_example_mixed}
\end{figure}


==> figure_symmetrization.tex <==
\begin{figure}
\begin{minipage}{.30\linewidth}
\begin{tikzpicture}

\draw[ultra thick] (0,0) -- (-1.00,-1.73) -- (1.00,-1.73) -- cycle;

\draw[dashed] (0,0) -- (-1.00,1.73);
\draw[dashed] (0,0) -- ( 1.00,1.73);

\draw ( 1.000,-1.730) -- ( 0.500,0.865) -- (-0.500,0.865) -- (-1.00,-1.730);
\draw ( 0.000, 0.000) -- ( 0.500,0.865);
\draw ( 0.000, 0.000) -- (-0.500,0.865);

\draw[-latex] (2,1) node[anchor=south west]{$\bb$} to[bend left] (0.1,0);

\draw (-1.00,-1.73) node[anchor=north east]{$\bc_-$};
\draw ( 1.00,-1.73) node[anchor=north west]{$\bc_+$};

\draw (-0.500, 0.865) node[anchor=east]{$\bc_-'$};
\draw ( 0.500, 0.865) node[anchor=west]{$\bc_+'$};

\draw[-latex] (0,2) node[anchor=south]{$\varepsilon$} to[bend left] (-0.2,0.5);

\end{tikzpicture}
\subcaption{}
\label{figure_patch_symmetrization_one}
\end{minipage}
\begin{minipage}{.30\linewidth}
\begin{tikzpicture}[scale=2]

\draw[ultra thick] (0,0) -- ({1.0*cos(   0)},{1.0*sin(   0)});
\draw[ultra thick] (0,0) -- ({1.1*cos(- 20)},{1.1*sin(- 20)});
\draw[ultra thick] (0,0) -- ({0.7*cos(- 60)},{0.7*sin(- 60)});
\draw[ultra thick] (0,0) -- ({1.3*cos(-140)},{1.3*sin(-140)});
\draw[ultra thick] (0,0) -- ({1.0*cos(-260)},{1.0*sin(-260)});

\draw[ultra thick] ({1.0*cos(   0)},{1.0*sin(   0)}) --
                   ({1.1*cos(- 20)},{1.1*sin(- 20)}) --
                   ({0.7*cos(- 60)},{0.7*sin(- 60)}) --
                   ({1.3*cos(-140)},{1.3*sin(-140)}) --
                   ({1.0*cos(-260)},{1.0*sin(-260)});

\draw[dashed] (0,0) -- ({1.5*cos( 0.38* 20)},{1.5*sin( 0.38* 20)});
\draw[dashed] (0,0) -- ({1.5*cos( 0.38* 60)},{1.5*sin( 0.38* 60)});
\draw[dashed] (0,0) -- ({1.5*cos( 0.38*140)},{1.5*sin( 0.38*140)});

\draw (0,0) -- ({0.8*cos( 0.38* 20)},{0.8*sin( 0.38* 20)});
\draw (0,0) -- ({0.8*cos( 0.38* 60)},{0.8*sin( 0.38* 60)});
\draw (0,0) -- ({0.8*cos( 0.38*140)},{0.8*sin( 0.38*140)});

\draw ({1.0*cos(        0)},{1.0*sin(        0)}) --
      ({0.8*cos( 0.38* 20)},{0.8*sin( 0.38* 20)}) --
      ({0.8*cos( 0.38* 60)},{0.8*sin( 0.38* 60)}) --
      ({0.8*cos( 0.38*140)},{0.8*sin( 0.38*140)}) --
      ({1.0*cos(-     260)},{1.0*sin(-     260)});

\draw[-latex] (0,1.5) node[anchor=south]{$\bb$} to[bend left] (0.025,0.1);

\draw ({1.0*cos(   0)},{1.0*sin(   0)}) node[anchor=west] {$\bc_+$} node[xshift=-1em, yshift=-0.75em] {$K_4$};
\draw ({1.1*cos(- 20)},{1.1*sin(- 20)}) node[anchor=west] {$\bd_3$} node[xshift=-2.5em] {$K_3$};
\draw ({0.7*cos(- 60)},{0.7*sin(- 60)}) node[anchor=north] {$\bd_2$} node[xshift=-3em, yshift=0.5em] {$K_2$};
\draw ({1.3*cos(-140)},{1.3*sin(-140)}) node[anchor=east] {$\bd_1$} node[xshift=3.5em, yshift=5em] {$K_1$};
\draw ({1.0*cos(-260)},{1.0*sin(-260)}) node[anchor=south] {$\bc_-$};

\draw ({0.8*cos( 0.38* 20)},{0.8*sin( 0.38* 20)}) node[anchor=south west] {$\bd_3'$} node[xshift=-0.5em, yshift=0.45em] {$\kappa_3$} node[xshift=-0.25em, yshift=-0.15em] {$\kappa_4$};
\draw ({0.8*cos( 0.38* 60)},{0.8*sin( 0.38* 60)}) node[anchor=south] {$\bd_2'$} node[xshift=-1.1em, yshift=0.25em] {$\kappa_2$};
\draw ({0.8*cos( 0.38*140)},{0.8*sin( 0.38*140)}) node[anchor=south] {$\bd_1'$} node[xshift=-1.85em, yshift=-0.5em] {$\kappa_1$};

\end{tikzpicture}
\subcaption{}
\label{figure_patch_symmetrization_several_close}
\end{minipage}
\begin{minipage}{.30\linewidth}
\begin{tikzpicture}[scale=2]

\draw[ultra thick] (0,0) -- ({1.0*cos(   0)},{1.0*sin(   0)});
\draw[ultra thick] (0,0) -- ({1.1*cos(- 20)},{1.1*sin(- 20)});
\draw[ultra thick] (0,0) -- ({0.5*cos(- 80)},{0.5*sin(- 80)});
\draw[ultra thick] (0,0) -- ({1.3*cos(-120)},{1.3*sin(-120)});

\draw[ultra thick] ({1.0*cos(   0)},{1.0*sin(   0)})
-- ({1.1*cos(- 20)},{1.1*sin(- 20)})
-- ({0.5*cos(- 80)},{0.5*sin(- 80)})
-- ({1.3*cos(-120)},{1.3*sin(-120)});

\draw[dashed] (0,0) -- ({2.0*cos(  2.0*20)},{2.0*sin(  2.0*20)});
\draw[dashed] (0,0) -- ({2.0*cos(  2.0*80)},{2.0*sin(  2.0*80)});

\draw         (0,0) -- ({0.5*cos(  2.0*20)},{0.5*sin(  2.0*20)});
\draw         (0,0) -- ({0.5*cos(  2.0*80)},{0.5*sin(  2.0*80)});

\draw         (1,0) -- ({0.5*cos(  2.0*20)},{0.5*sin(  2.0*20)}) -- ({0.5*cos(  2.0*80)},{0.5*sin(  2.0*80)}) -- ({1.3*cos(-120)},{1.3*sin(-120)});

\draw ({0.5*cos(  2.0*20)},{0.5*sin(  2.0*20)}) node[anchor=south] {$\bd_2'$} node[xshift=-2em, yshift=-1em] {$\kappa_2$} node[xshift=0.15em, yshift=-0.95em] {$\kappa_3$};
\draw ({0.5*cos(  2.0*80)},{0.5*sin(  2.0*80)}) node[anchor=south] {$\bd_1'$} node[xshift=0.55em, yshift=-2em] {$\kappa_1$};
\draw ({1.1*cos(- 20)},{1.1*sin(- 20)}) node[anchor=north] {$\bd_2$} node[xshift=-3.5em, yshift=0.5em] {$K_2$};
\draw ({0.5*cos(- 80)},{0.5*sin(- 80)}) node[anchor=north] {$\bd_1$} node[xshift=-0.7em, yshift=0.5em] {$K_1$};

\draw ({1.0*cos(   0)},{1.0*sin(   0)}) node[anchor=west] {$\bc_+$} node[xshift=-1em, yshift=-0.75em] {$K_3$};
\draw ({1.3*cos(-120)},{1.3*sin(-120)}) node[anchor=east] {$\bc_-$};

\draw[-latex] (-1,1) node[anchor=south east]{$\bb$} to[bend left] (0,0.1);
\draw[-latex] (-1,-0.25) node[anchor=east]{$\varepsilon$} to[bend right] (-0.25,0.05);

\end{tikzpicture}
\subcaption{}
\label{figure_patch_symmetrization_several_open}
\end{minipage}
\caption{Extensions around problematic vertices}
\label{figure_patch_symmetrization}
\end{figure}



==> figures/figure_extension.tex <==
\begin{figure}

\begin{tikzpicture}[scale=3]

\draw (0,-1) -- (0,1) -- (-1.73205080756887729352,0) -- cycle;

\draw[dotted] (0,1) -- (1.73205080756887729352/2,1/2) -- (1.73205080756887729352/2,-1/2) -- (0,-1);

\draw[dotted] (0,-1) -- (1.73205080756887729352/2,1/2); 
\draw[dotted] (1.73205080756887729352/2,-1/2) -- (0,1);

\draw (-1.73205080756887729352/2,0) node {$K$};

\draw (0.25, 0.0) node {$\widetilde K_1$};
\draw (0.50, 0.5) node {$\widetilde K_2$};
\draw (0.75, 0.0) node {$\widetilde K_3$};
\draw (0.50,-0.5) node {$\widetilde K_4$};

\draw (-1.73205080756887729352,0) node[anchor=east] {$\bc$};

\draw (0, 1) node[anchor=south] {$\bb_-$};
\draw (0,-1) node[anchor=north] {$\bb_+$};

\draw (1.73205080756887729352/2, 1/2) node[anchor=south west] {$\widetilde \bb_+$}; 
\draw (1.73205080756887729352/2,-1/2) node[anchor=north west] {$\widetilde \bb_-$};

\draw[->] (1,1) edge[bend right] (1.73205080756887729352/3,0);

\draw (1,1) node[anchor=west] {$\widetilde \bc$};

\end{tikzpicture}

\caption{Extension of tetrahedra with boundary faces}
\label{figure_extension}
\end{figure}


==> figures/figure_mixed_patches.tex <==
\tikzset{math3d/.style=
{x= {(-0.353cm,-0.353cm)}, z={(0cm,1.3cm)},y={(0.0cm,0.7cm)}}}
%{x= {(-0.5cm,-0.5cm)}, z={(0cm,1.0cm)},y={(0.0cm,0.5cm)}}}

\begin{figure}
\def\sz{0.65}
\def\sza{0.45}
\def\opac{1}

\begin{minipage}{.45\linewidth}
\centering
\begin{tikzpicture}[math3d, scale=3.3]
%filled faces
\fill[color=gray!20] (0,0, 1) -- (-1,-1,0) -- (0,0,0) -- cycle;
\fill[color=gray!20] (0,0,-1) -- (-1,-1,0) -- (0,0,0) -- cycle;
\fill[color=gray!20] (0,0, 1) -- ( 1, 1,0) -- (0,0,0) -- cycle;
\fill[color=gray!80] (0,0,-1) -- ( 1, 1,0) -- (0,0,0) -- cycle;

%edges
\draw[        line width=\sz pt] (-1,-1,0)--(0,0,0)--(1,1,0);

\draw[        line width=\sz pt] ( 0, 0, 0) -- ( 0, 0, 1);

\draw[dashed, line width=\sz pt] ( 1, 1, 0) -- (-1, 0, 0);
\draw[        line width=\sz pt] (-1,-1, 0) -- (-1, 0, 0);
\draw[        line width=\sz pt] ( 0, 0, 1) -- (-1, 0, 0);
\draw[dashed, line width=\sz pt] ( 0, 0, 0) -- (-1, 0, 0);
\draw[dashed, line width=\sz pt] ( 0, 0,-1) -- (-1, 0, 0);

\draw[        line width=\sz pt] ( 0, 0, 1) -- ( 1, 1, 0);
\draw[        line width=\sz pt] ( 0, 0, 1) -- (-1,-1, 0);

\draw[        line width=\sz pt] ( 0, 0, 0) -- ( 0, 0,-1);
\draw[        line width=\sz pt] ( 0, 0,-1) -- ( 1, 1, 0);
\draw[        line width=\sz pt] ( 0, 0,-1) -- (-1,-1, 0);
\end{tikzpicture}
\end{minipage}
\begin{minipage}{.45\linewidth}
\centering
\begin{tikzpicture}[math3d, scale=3.3]
%filled faces
\fill[color=gray!20] (-1, 0, 0) -- (-1, 0,-1) -- (0,0,0) -- cycle;
\fill[color=gray!20] ( 0, 0,-1) -- (-1, 0,-1) -- (0,0,0) -- cycle;
\fill[color=gray!80] ( 0, 0,-1) -- ( 1, 1, 0) -- (0,0,0) -- cycle;
\fill[color=gray!20] (-1, 0, 0) -- ( 1, 1, 0) -- (0,0,0) -- cycle;

\draw[line width=\sz pt] (-1, 0, 0) -- (-1, 0,-1) -- (0,0,0) -- cycle;
\draw[line width=\sz pt] ( 0, 0,-1) -- (-1, 0,-1) -- (0,0,0) -- cycle;
\draw[line width=\sz pt] ( 0, 0,-1) -- ( 1, 1, 0) -- (0,0,0) -- cycle;
\draw[line width=\sz pt] (-1, 0, 0) -- ( 1, 1, 0) -- (0,0,0) -- cycle;

\draw[dashed,line width=\sz pt] (-1, 0, 0) -- (-0.3,1,-1);
\draw[dashed,line width=\sz pt] ( 0, 0,-1) -- (-0.3,1,-1);
\draw[dashed,line width=\sz pt] ( 0, 0,-1) -- (-0.3,1,-1);
\draw[dashed,line width=\sz pt] (-1, 0, 0) -- (-0.3,1,-1);

\draw[dashed,line width=\sz pt] (-1, 0,-1) -- (-0.3,1,-1);
\draw[dashed,line width=\sz pt] (-1, 0,-1) -- (-0.3,1,-1);
\draw[dashed,line width=\sz pt] ( 1, 1, 0) -- (-0.3,1,-1);
\draw[dashed,line width=\sz pt] ( 1, 1, 0) -- (-0.3,1,-1);

\draw[dashed,line width=\sz pt] ( 0, 0, 0) -- (-0.3,1,-1);
\end{tikzpicture}
\end{minipage}

\caption{Example of patches with mixed boundary conditions covered by our analysis.
\cblue{The patch on the left is not immediately covered, but can be transformed
into the patch on the right. If either the dark grey boundary correspond to $\Ga$
(and thus, the light grey is $\FDa$) or if the light grey represents
$\Ga$ (and the dark grey, $\FDa$), then the patch on the right is covered in
Example \ref{example_corner}.}}
\label{figure_example_mixed}
\end{figure}


==> figures/figure_symmetrization.tex <==
\begin{figure}
\begin{minipage}{.30\linewidth}
\begin{tikzpicture}

\draw[ultra thick] (0,0) -- (-1.00,-1.73) -- (1.00,-1.73) -- cycle;

\draw[dashed] (0,0) -- (-1.00,1.73);
\draw[dashed] (0,0) -- ( 1.00,1.73);

\draw ( 1.000,-1.730) -- ( 0.500,0.865) -- (-0.500,0.865) -- (-1.00,-1.730);
\draw ( 0.000, 0.000) -- ( 0.500,0.865);
\draw ( 0.000, 0.000) -- (-0.500,0.865);

\draw[-latex] (2,1) node[anchor=south west]{$\bb$} to[bend left] (0.1,0);

\draw (-1.00,-1.73) node[anchor=north east]{$\bc_-$};
\draw ( 1.00,-1.73) node[anchor=north west]{$\bc_+$};

\draw (-0.500, 0.865) node[anchor=east]{$\bc_-'$};
\draw ( 0.500, 0.865) node[anchor=west]{$\bc_+'$};

\draw[-latex] (0,2) node[anchor=south]{$\varepsilon$} to[bend left] (-0.2,0.5);

\end{tikzpicture}
\subcaption{}
\label{figure_patch_symmetrization_one}
\end{minipage}
\begin{minipage}{.30\linewidth}
\begin{tikzpicture}[scale=2]

\draw[ultra thick] (0,0) -- ({1.0*cos(   0)},{1.0*sin(   0)});
\draw[ultra thick] (0,0) -- ({1.1*cos(- 20)},{1.1*sin(- 20)});
\draw[ultra thick] (0,0) -- ({0.7*cos(- 60)},{0.7*sin(- 60)});
\draw[ultra thick] (0,0) -- ({1.3*cos(-140)},{1.3*sin(-140)});
\draw[ultra thick] (0,0) -- ({1.0*cos(-260)},{1.0*sin(-260)});

\draw[ultra thick] ({1.0*cos(   0)},{1.0*sin(   0)}) --
                   ({1.1*cos(- 20)},{1.1*sin(- 20)}) --
                   ({0.7*cos(- 60)},{0.7*sin(- 60)}) --
                   ({1.3*cos(-140)},{1.3*sin(-140)}) --
                   ({1.0*cos(-260)},{1.0*sin(-260)});

\draw[dashed] (0,0) -- ({1.5*cos( 0.38* 20)},{1.5*sin( 0.38* 20)});
\draw[dashed] (0,0) -- ({1.5*cos( 0.38* 60)},{1.5*sin( 0.38* 60)});
\draw[dashed] (0,0) -- ({1.5*cos( 0.38*140)},{1.5*sin( 0.38*140)});

\draw (0,0) -- ({0.8*cos( 0.38* 20)},{0.8*sin( 0.38* 20)});
\draw (0,0) -- ({0.8*cos( 0.38* 60)},{0.8*sin( 0.38* 60)});
\draw (0,0) -- ({0.8*cos( 0.38*140)},{0.8*sin( 0.38*140)});

\draw ({1.0*cos(        0)},{1.0*sin(        0)}) --
      ({0.8*cos( 0.38* 20)},{0.8*sin( 0.38* 20)}) --
      ({0.8*cos( 0.38* 60)},{0.8*sin( 0.38* 60)}) --
      ({0.8*cos( 0.38*140)},{0.8*sin( 0.38*140)}) --
      ({1.0*cos(-     260)},{1.0*sin(-     260)});

\draw[-latex] (0,1.5) node[anchor=south]{$\bb$} to[bend left] (0.025,0.1);

\draw ({1.0*cos(   0)},{1.0*sin(   0)}) node[anchor=west] {$\bc_+$} node[xshift=-1em, yshift=-0.75em] {$K_4$};
\draw ({1.1*cos(- 20)},{1.1*sin(- 20)}) node[anchor=west] {$\bd_3$} node[xshift=-2.5em] {$K_3$};
\draw ({0.7*cos(- 60)},{0.7*sin(- 60)}) node[anchor=north] {$\bd_2$} node[xshift=-3em, yshift=0.5em] {$K_2$};
\draw ({1.3*cos(-140)},{1.3*sin(-140)}) node[anchor=east] {$\bd_1$} node[xshift=3.5em, yshift=5em] {$K_1$};
\draw ({1.0*cos(-260)},{1.0*sin(-260)}) node[anchor=south] {$\bc_-$};

\draw ({0.8*cos( 0.38* 20)},{0.8*sin( 0.38* 20)}) node[anchor=south west] {$\bd_3'$} node[xshift=-0.5em, yshift=0.45em] {$\kappa_3$} node[xshift=-0.25em, yshift=-0.15em] {$\kappa_4$};
\draw ({0.8*cos( 0.38* 60)},{0.8*sin( 0.38* 60)}) node[anchor=south] {$\bd_2'$} node[xshift=-1.1em, yshift=0.25em] {$\kappa_2$};
\draw ({0.8*cos( 0.38*140)},{0.8*sin( 0.38*140)}) node[anchor=south] {$\bd_1'$} node[xshift=-1.85em, yshift=-0.5em] {$\kappa_1$};

\end{tikzpicture}
\subcaption{}
\label{figure_patch_symmetrization_several_close}
\end{minipage}
\begin{minipage}{.30\linewidth}
\begin{tikzpicture}[scale=2]

\draw[ultra thick] (0,0) -- ({1.0*cos(   0)},{1.0*sin(   0)});
\draw[ultra thick] (0,0) -- ({1.1*cos(- 20)},{1.1*sin(- 20)});
\draw[ultra thick] (0,0) -- ({0.5*cos(- 80)},{0.5*sin(- 80)});
\draw[ultra thick] (0,0) -- ({1.3*cos(-120)},{1.3*sin(-120)});

\draw[ultra thick] ({1.0*cos(   0)},{1.0*sin(   0)})
-- ({1.1*cos(- 20)},{1.1*sin(- 20)})
-- ({0.5*cos(- 80)},{0.5*sin(- 80)})
-- ({1.3*cos(-120)},{1.3*sin(-120)});

\draw[dashed] (0,0) -- ({2.0*cos(  2.0*20)},{2.0*sin(  2.0*20)});
\draw[dashed] (0,0) -- ({2.0*cos(  2.0*80)},{2.0*sin(  2.0*80)});

\draw         (0,0) -- ({0.5*cos(  2.0*20)},{0.5*sin(  2.0*20)});
\draw         (0,0) -- ({0.5*cos(  2.0*80)},{0.5*sin(  2.0*80)});

\draw         (1,0) -- ({0.5*cos(  2.0*20)},{0.5*sin(  2.0*20)}) -- ({0.5*cos(  2.0*80)},{0.5*sin(  2.0*80)}) -- ({1.3*cos(-120)},{1.3*sin(-120)});

\draw ({0.5*cos(  2.0*20)},{0.5*sin(  2.0*20)}) node[anchor=south] {$\bd_2'$} node[xshift=-2em, yshift=-1em] {$\kappa_2$} node[xshift=0.15em, yshift=-0.95em] {$\kappa_3$};
\draw ({0.5*cos(  2.0*80)},{0.5*sin(  2.0*80)}) node[anchor=south] {$\bd_1'$} node[xshift=0.55em, yshift=-2em] {$\kappa_1$};
\draw ({1.1*cos(- 20)},{1.1*sin(- 20)}) node[anchor=north] {$\bd_2$} node[xshift=-3.5em, yshift=0.5em] {$K_2$};
\draw ({0.5*cos(- 80)},{0.5*sin(- 80)}) node[anchor=north] {$\bd_1$} node[xshift=-0.7em, yshift=0.5em] {$K_1$};

\draw ({1.0*cos(   0)},{1.0*sin(   0)}) node[anchor=west] {$\bc_+$} node[xshift=-1em, yshift=-0.75em] {$K_3$};
\draw ({1.3*cos(-120)},{1.3*sin(-120)}) node[anchor=east] {$\bc_-$};

\draw[-latex] (-1,1) node[anchor=south east]{$\bb$} to[bend left] (0,0.1);
\draw[-latex] (-1,-0.25) node[anchor=east]{$\varepsilon$} to[bend right] (-0.25,0.05);

\end{tikzpicture}
\subcaption{}
\label{figure_patch_symmetrization_several_open}
\end{minipage}
\caption{Extensions around problematic vertices}
\label{figure_patch_symmetrization}
\end{figure}


